Heta: Distributed Training of Heterogeneous Graph Neural Networks

Heterogeneous Graph Neural Networks (HGNNs) leverage diverse semantic relationships in Heterogeneous Graphs (HetGs) and have demonstrated remarkable learning performance in various applications. However, current distributed GNN training systems often overlook unique characteristics of HetGs, such as varying feature dimensions and the prevalence of missing features among nodes, leading to suboptimal performance or even incompatibility with distributed HGNN training. We introduce Heta, a framework designed to address the communication bottleneck in distributed HGNN training. Heta leverages the inherent structure of HGNNs - independent relation-specific aggregations for each relation, followed by a cross-relation aggregation - and advocates for a novel Relation-Aggregation-First computation paradigm. It performs relation-specific aggregations within graph partitions and then exchanges partial aggregations. This design, coupled with a new graph partitioning method that divides a HetG based on its graph schema and HGNN computation dependency, substantially reduces communication overhead. Heta further incorporates an innovative GPU feature caching strategy that accounts for the different cache miss-penalties associated with diverse node types. Comprehensive evaluations of various HGNN models and large heterogeneous graph datasets demonstrate that Heta outperforms state-of-the-art systems like DGL and GraphLearn by up to 5.8x and 2.3x in end-to-end epoch time, respectively.

==> discussions.tex <==
\section{Discussions}
\label{sec:discussions}



The meta-partitioning algorithm brings several benefits. 

\vspace{1mm}
\noindent\textbf{Reduce communication overhead.} After the partitioning process, the boundary nodes are restricted to nodes of the target node type. The partitions are largely self-reliant, as all operations can be executed locally, with the exception of the boundary nodes. These boundary nodes necessitate an $\text{AGG}_{\text{all}}$ operation to aggregate partial aggregations from other partitions. Our method enables workers to perform graph sampling, feature fetching, and partial aggregations locally, eliminating the need for communication with other machines. The communication required for aggregating partial aggregations (and their backward gradients) for boundary nodes is minimal. For example, for the ogbn-mag dataset~\cite{hu2020open}, the number of boundary nodes (i.e., target node type `paper`) is 7.4 millions, and the size of partial aggregations (assume hidden dimension is 64) to communicate amounts to only 188MB per training epoch for each machine. Conversely, 
when utilizing DGL with METIS partitioning on two partitions, fetching features from remote machines for the ogbn-mag dataset during each training epoch requires XX GB. Note that this amount is several orders of magnitude greater than what our method entails. Additionally, in our case, the communication volume and the fanout and layers of the sample layer are independent of each other. They are solely determined by the number of training nodes and remain constant. However, systems like DGL necessitate higher communication volume when employing larger fanouts or deeper layers, as they require a greater number of neighbors for feature fetching.


\vspace{1mm}
\noindent\textbf{Fast and efficient.} The technique of meta-partitioning operates exclusively on the metagraph rather than on specific nodes and edges. This characteristic contributes to its high efficiency. The metagraph is significantly smaller than its corresponding HetG, which may contain millions of nodes and billions of edges. In contrast, the metagraph consists of only a few nodes and edges. When considering the number of node types, denoted as $|A|$, and edge types, denoted as $|R|$, the complexity of a BFS algorithm is at most $O(|R|)$ when it traverses all edges. Additionally, since there can be at most $|A|$ sub-metatrees (in the scenario where all node types are connected to the target node type), the time complexity for sorting and deduplication is $O(|A| \log |A|)$. Therefore, the overall time complexity is $O(|A| \log |A|) + O(|R|)$. Traditional graph partitioning algorithms, which consider specific nodes, typically have a time complexity of at least $O(|V|)$, where $|V|$ represents the number of nodes in the graph~\cite{bulucc2016recent}. Note that $|V| \gg |A|$ and $|V| \gg |R|$. The subsequent experiments conducted also confirm the swift performance of meta-partitioning, as demonstrated in Table~\ref{tab:partition_comparison}.


\vspace{1mm}
\noindent\textbf{Improve cache hit rate with partition-aware cache.} Meta-partitioning offers an additional advantage: improving the cache hit rate of the GPU feature cache. As described in \S\ref{sec:challenges}, in order to tackle the communication bottleneck, previous works have proposed using the GPU cache to cache the features of the most visited nodes~\cite{lin2020pagraph, yang2022gnnlab, sun2023legion}.
With meta-partitioning, each partition contains only a subset of node types, rather than all of them. Consequently, we only cache node features or learnable features for the node types present within each partition. This approach is referred to as partition-aware cache. 
Without meta-partitioning, the ``cache space'' is large, which is the nodes of the entire graph. Each GPU worker samples from the whole graph, resulting in sampled subgraphs that contain all types of nodes from the whole graph. But with meta-partitioning and partition-aware cache, the ``cache space'' is confined to the local partition (part of the graph), thereby leading to a higher cache hit rate. 
As demonstrated in Figure~\ref{fig:cache_space}, following the example from Figure~\ref{fig:meta_partitioning_workflow}, if there were no meta-partitioning, the ``cache space'' for each partition would encompass the entire graph. However, with meta-partitioning, the leaf nodes for Partition 1 are P (Paper) and I (Institution), whereas for Partition 2, they are A (Author) and F (Field of Study). Therefore, the ``cache space '' is significantly reduced. As a result, the cache hit rate markedly improves due to the confined node types. The subsequent experiment also validate this, as shown in Table XX. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/cache_space.pdf}
    \caption{The cache space with or without meta-partitioning.}
    \vspace{-3mm}
    \label{fig:cache_space}
\end{figure}





